Incremental Dense Reconstruction from Monocular Video with Guided Sparse Feature Volume Fusion

Incrementally recovering 3D dense structures from monocular videos is of paramount importance since it enables various robotics and AR applications. Feature volumes have recently been shown to enable efficient and accurate incremental dense reconstruction without the need to first estimate depth, but they are not able to achieve as high of a resolution as depth-based methods due to the large memory consumption of high-resolution feature volumes. This letter proposes a real-time feature volume-based dense reconstruction method that predicts TSDF (Truncated Signed Distance Function) values from a novel sparsified deep feature volume, which is able to achieve higher resolutions than previous feature volume-based methods, and is favorable in large-scale outdoor scenarios where the majority of voxels are empty. An uncertainty-aware multi-view stereo (MVS) network is leveraged to infer initial voxel locations of the physical surface in a sparse feature volume. Then for refining the recovered 3D geometry, deep features are attentively aggregated from multiview images at potential surface locations, and temporally fused. Besides achieving higher resolutions than before, our method is shown to produce more complete reconstructions with finer detail in many cases. Extensive evaluations on both public and self-collected datasets demonstrate a very competitive real-time reconstruction result for our method compared to state-of-the-art reconstruction methods in both indoor and outdoor settings.

==> figures/meshes.tex <==
\begin{figure*} [t]
	% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\newcommand{\w}{.14\textwidth}
	\centering
	\foreach \method/\stamp in {GPMVS~\cite{hou2019multi}/snapshot00_L01.png, Atlas~\cite{murez2020atlas}/snapshot00_L02.png, Vortx~\cite{stier2021vortx}/snapshot00_L03.png, NeuralRecon~\cite{sun2021neuralrecon}/snapshot00_L04.png, Ours/snapshot00_L05.png, Ours-High/snapshot00_L06.png, Gt/snapshot00_L00.png} {
		\begin{subfigure}[t]{\w}
			%& \begin{minipage}[c]{\w}\centering
			\caption*{\textbf{\method}}
			\includegraphics[width=\columnwidth]{%
				figures/shownmesh/scene0806_00/\stamp} 
			%  \end{minipage}
		\end{subfigure} \hspace{-9pt}
	}  
	
	\centering
	\foreach \stamp in {snapshot00_L01.png, snapshot00_L02.png, snapshot00_L03.png, snapshot00_L04.png, snapshot00_L05.png, snapshot00_L06.png, snapshot00_L00.png} {
		\begin{subfigure}[t]{\w}
			%& \begin{minipage}[c]{\w}\centering
			\includegraphics[width=\columnwidth]{%
				figures/shownmesh/scene0801_00/\stamp} 
			%  \end{minipage}
		\end{subfigure} \hspace{-9pt}
	}  
	
	
	% Row 2. Separate to put the space for line break
	\centering
	\foreach \stamp in {snapshot00_L01.png, snapshot00_L02.png, snapshot00_L03.png, snapshot00_L04.png, snapshot00_L05.png, snapshot00_L06.png, snapshot00_L00.png} {
		\begin{subfigure}[t]{\w}
			%& \begin{minipage}[c]{\w}\centering
			\includegraphics[width=\columnwidth]{%
				figures/shownmesh/scene0750_00/\stamp} 
			%  \end{minipage}
		\end{subfigure} \hspace{-9pt}
	} 
	
	% Row 3. Separate to put the space for line break
	\centering
	\foreach \stamp in {snapshot00_L01.png, snapshot00_L02.png, snapshot00_L03.png, snapshot00_L04.png, snapshot00_L05.png, snapshot00_L06.png, snapshot00_L00.png} {
		\begin{subfigure}[t]{\w}
			%& \begin{minipage}[c]{\w}\centering
			\includegraphics[width=\columnwidth]{%
				figures/shownmesh/scene0714_00/\stamp} 
			%  \end{minipage}
		\end{subfigure} \hspace{-9pt}
	}
	
	% Row 4. Separate to put the space for line break
	\centering
	\foreach \stamp in {snapshot00_L01.png, snapshot00_L02.png, snapshot00_L03.png, snapshot00_L04.png, snapshot00_L05.png, snapshot00_L06.png, snapshot00_L00.png} {
		\begin{subfigure}[t]{\w}
			%& \begin{minipage}[c]{\w}\centering
			\includegraphics[width=\columnwidth]{%
				figures/shownmesh/scene0710_00/\stamp} 
			%  \end{minipage}
		\end{subfigure} \hspace{-9pt}
	}
	
	% Row 5. Separate to put the space for line break
	\centering
	\foreach \stamp in {snapshot00_L01.png, snapshot00_L02.png, snapshot00_L03.png, snapshot00_L04.png, snapshot00_L05.png, snapshot00_L06.png, snapshot00_L00.png} {
		\begin{subfigure}[t]{\w}
			%& \begin{minipage}[c]{\w}\centering
			\includegraphics[width=\columnwidth]{%
				figures/shownmesh/scene0721_00/\stamp} 
			%  \end{minipage}
		\end{subfigure} \hspace{-9pt}
	}
	
	% Row 6. Separate to put the space for line break
	\centering
	\foreach \stamp in {snapshot00_L01.png, snapshot00_L02.png, snapshot00_L03.png, snapshot00_L04.png, snapshot00_L05.png, snapshot00_L06.png, snapshot00_L00.png} {
		\begin{subfigure}[t]{\w}
			%& \begin{minipage}[c]{\w}\centering
			\includegraphics[width=\columnwidth]{%
				figures/shownmesh/scene0761_00/\stamp} 
			%  \end{minipage}
		\end{subfigure} \hspace{-9pt}
	} 
	
	% Row 6. Separate to put the space for line break
	\centering
	\foreach \stamp in {snapshot00_L01.png, snapshot00_L02.png, snapshot00_L03.png, snapshot00_L04.png, snapshot00_L05.png, snapshot00_L06.png, snapshot00_L00.png} {
		\begin{subfigure}[t]{\w}
			%& \begin{minipage}[c]{\w}\centering
			\includegraphics[width=\columnwidth]{%
				figures/shownmesh/scene0787_00/\stamp} 
			%  \end{minipage}
		\end{subfigure} \hspace{-9pt}
	} 
	
	% Row 6. Separate to put the space for line break
	\centering
	\foreach \seq/\stamp in {snapshot00_L01.png, snapshot00_L02.png, snapshot00_L03.png, snapshot00_L04.png, snapshot00_L05.png, snapshot00_L06.png, snapshot00_L00.png} {
		\begin{subfigure}[t]{\w}
			%& \begin{minipage}[c]{\w}\centering
			\includegraphics[width=\columnwidth]{%
				figures/shownmesh/scene0747_00/\stamp} 
			%  \end{minipage}
		\end{subfigure} \hspace{-9pt}
	} 
	
	%\vspace{-1em}
	\caption{
		Some qualitative results from the Scannet Dataset.
	}
	%\end{tabular}
	\vspace{-2em}
	\label{fig:meshes}
\end{figure*}



==> figures/showmesh_realsense/06-11-2022-16-54-28/tmp-pdfcrop-40019.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{677430312E706466}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{3}


==> sections_main/01_abstract.tex <==
%!TEX root = ../main.tex

\begin{abstract}
%
\rev{Incrementally recovering 3D dense structures from monocular videos is of paramount importance since it enables various robotics and AR applications.}
%
Feature volumes have recently been shown to enable efficient and accurate incremental dense reconstruction without the need to first estimate depth, but they are not able to achieve as high of a resolution as depth-based methods due to the large memory consumption of high-resolution feature volumes.
%
This letter proposes a real-time feature volume-based dense reconstruction method that predicts TSDF (Truncated Signed Distance Function) values from a novel {\em sparsified} deep feature volume, which is able to achieve higher resolutions than previous feature volume-based methods, \rev{and is favorable in outdoor large-scale scenarios where the majority of voxels are empty}.
%
An uncertainty-aware multi-view stereo (MVS) network is leveraged to infer initial voxel locations of the physical surface in a sparse feature volume.
Then for refining the recovered 3D geometry, deep features are attentively aggregated from multi-view images at potential surface locations, and temporally fused. % with GRU (Gated Recurrent Unit) fusion. 
%
%With simple MLP (Multi-layer Perceptrons) layers, we are able to predict TSDF values from the sparse feature volumes for a coherent surface reconstruction.
%
%The sparse feature volume guided by MVS is memory efficient, and makes the high-resolution feature-volume-based reconstruction applicable.
%
Besides achieving higher resolutions than before, %our use of MVS depth to guide the feature volume allocation also allows the network 
our method is shown to produce more complete reconstructions with finer detail in many cases.
%\rev{Taking into account the sparsity of 3D space, our method is able to generalize more effectively for outdoor large-scale scenarios.}
Extensive evaluations on both public \rev{and self-collected datasets} demonstrate a very competitive real-time reconstruction result for our method compared to state-of-the-art reconstruction methods \rev{in both indoor and outdoor settings}.
%
\end{abstract}

%%================================================
%% FOR RAL JOURNAL
%%================================================
\begin{IEEEkeywords}
 Monocular Dense Mapping, Neural Implicit Representation, Feature Volume Fusion
\end{IEEEkeywords}
%%================================================
%%================================================


==> sections_main/02_intro_relawork.tex <==
%!TEX root = ../main.tex

\begin{figure*} %[!t]
	\centering
%	\includegraphics[width=\textwidth,height=0.25\textheight]{figures/framework_incremental2.png}
 	\includegraphics[width=0.9\textwidth]{figures/framework_incremental3_s}
	\caption{ The overview of our proposed method. We leverage \rev{an} MVS neural network for depth and depth uncertainty predictions, which provide an initial guess of the physical surface location. Then feature volume-based reconstruction pipeline allocate and aggregate deep features around the physical surface, formatting sparse feature volume. TSDF values can be directly regressed from the feature volume which is incrementally updated. \rev{Note that the pipeline involves three levels of feature volumes, which are omitted here for simplicity.}
    % for a fragment of images. 3D sparse CNN and GRU fusion are conducted to incrementally fuse fragment feature volumes into a global one. TSDF values can be directly regressed from the global feature volume for an increment and coherent dense reconstruction.
   }
	\label{fig:framework}
	\vspace*{-2em}
\end{figure*}

\section{Introduction}
%
\IEEEPARstart{D}{ense} reconstruction from video images with deep neural networks has attracted significant attention in recent years. Deep feature volume-based 3D scene reconstruction, regressing scene geometry directly from volumetric feature volume, has shown promising results~\cite{murez2020atlas, sun2021neuralrecon, bozic2021transformerfusion, stier2021vortx}, and has the potential to enable a wide range of robotic applications. The incremental variant~\cite{sun2021neuralrecon} can even achieve real-time performance on a desktop with commercial-level GPU.
%
Compared to predicting dense depth at multiple views and then fusing depths into a global 3D map, feature volume-based method back-project encoded 2D image features into 3D voxel grids, and directly regress truncated signed distance function (TSDF) from accumulated features across multiple image views, by using \rev{a} neural network composed of 3D convolutional layers and multiple layer perceptron (MLP) layers. Operation and prediction directly on the view-independent 3D feature volume have the advantage of capturing smoothness and 3D shape prior of the surface in the scene.
%
% \rev{Feature volume-based dense reconstruction has the potential to enable a wide range of robotic applications. The volumetric TSDF map regressed from the features can be readily transformed into an occupancy map, which is crucial for various tasks such as obstacle avoidance, path planning, and autonomous navigation.}

 However, there are several drawbacks for existing feature volume-based methods~\cite{murez2020atlas, sun2021neuralrecon, bozic2021transformerfusion, stier2021vortx}.
% Back-projection along the whole ray
Firstly, allocating features into all visible voxels along the whole rays cast from image pixels is cumbersome and redundant, which not only creates unnecessary confusion for network inference but also incurs excessive memory consumption and heavy computational burden. The ideal solution is only allocating image features into the relevant regions in 3D space, i.e., around the physical surface, for reconstruction. In the case that surface location is not certainly known, features can be allocated to the potential region where the surface is likely to locate.
% Limited scale and resolution % and large-scale scenes
Secondly, due to the memory and computation issue for the volumetric dense feature volume, existing methods~\cite{murez2020atlas, sun2021neuralrecon, bozic2021transformerfusion, stier2021vortx} are not capable of high-resolution reconstruction.
% \rev{and limited to work in room-scale indoor scenarios}. 
All of them have demonstrated to ability to perform 3D dense reconstruction with feature volume, using a voxel size of over 4cm at the finest level. It is acceptable but causes visible aliasing artifacts \rev{such as surfaces appearing overly smooth and lacking fine details.} Besides, the memory consumption of feature volume  grows cubically with the increased volumetric resolution, which hinders existing methods from scaling up to high-resolution and fine-detailed reconstruction. 
%Higher resolution also requires more features in voxel grids need to be fed into subsequent 3D convolutions and MLPs, which further increases the computational burden.  
% Features with equal weight
% Thirdly, treating image features across different views allocated in a voxel equally without considering the relevance of features to the specific voxel location is not optimal.

To address the aforementioned issues, we propose a novel guided sparse feature volume fusion method for real-time incremental scene reconstruction. 
% In this paper, we focus on real-time incremental scene reconstruction based on feature volume.
Feature volumes are constructed fragment by fragment, and temporally fused into a global one. This incremental paradigm frequently updates the reconstructed 3D map, which favors real-time applications.
To maintain the sparsity of the feature volume for efficient reconstruction, we propose a method to selectively allocate features into only relevant voxels around the actual physical surface, which aims to avoid excessive memory and computation consumption. We firstly leverage an efficient MVS network to predict dense depth and depth uncertainty, which is used to select the sparse set of voxels to be aggregated for predicting the surface.
%With the predicted depth and uncertainty for every image in the fragment, image features from multi-views are allocated into the voxels at potential locations. 
%
A self-attention mechanism~\cite{vaswani2017attention} is utilized for feature aggregations across multiple views,
%
and then 3D sparse convolutions are performed on the feature volume, followed by Gated Recurrent Unit (GRU)~\cite{chung2014empirical} to temporally fuse the feature volume fragment into the global one.
We also utilize traditional TSDF fusion~\cite{newcombe2011kinectfusion} with the available depths from MVS to generate a rough TSDF map, which is used as an additional feature channel to guide the feature volume-based reconstruction. The contribution of this paper can be summarized as follows:
\begin{itemize}
	\item We develop a real-time incremental reconstruction system for monocular video images based on novel sparse feature volume fusion.   
	\item We propose to utilize MVS neural networks to predict initial depth and depth uncertainty maps for efficient feature allocation into 3D voxels, which maintains the natural sparsity of the problem and allows our method to recover more fine-grained details and \rev{to work effectively in outdoor large-scale scenarios}. 
    %Due to the sparsity, our method is memory-efficient and enables high-resolution scene reconstruction.
	\item The proposed method is verified on various datasets, and demonstrated to have
    %memory-efficient to attain high-resolution and accurate reconstruction.  The proposed method is realtime capable and has 
    competitive reconstruction accuracy compared to state-of-the-art methods, 
    and able to predict at a higher resolution than previous feature volume-based methods.
	% The accuracy of the reconstructed surfaces outperform existing feature-volume-based methods.
\end{itemize}

\iffalse
In what follows, after first discussing some related works, we present our proposed methodology in Section
\ref{sec:methodology}. Firstly, we overview the whole reconstruction pipeline. Then the MVS-guided sparse feature volume generation method is presented in detail. We further discuss the fragment reconstruction based on sparse feature volume, and disclose some implementation details. In Section~\ref{sec:exp}, we conduct thorough evaluations of the method on publicly-available datasets, comparing against state-of-the-art baselines. Finally, in Section~\ref{sec:conc} we summarize our results and
findings, and briefly discuss some potential future extensions of this work.
\fi

\section{Related Work}

Dense reconstruction from monocular videos has become increasingly accurate and robust with the emergence of deep learning. Our work is relevant to multi-view stereo (MVS) networks and feature volume-based scene reconstruction.

%\noindent\textbf
\subsection{Depth-based Reconstruction with MVS Networks.}
% MVS
Given a set of monocular images with known poses and camera intrinsics, the goal of MVS networks is to infer the dense depth map of the reference frame using the provided multi-view information. 
%
Inspired by traditional plane-sweeping MVS methods~\cite{collins1996space},  a rich body of MVS neural networks first construct a plane-sweeping cost volume using the image intensity values~\cite{wang2018mvdepthnet, hou2019multi} or deep 2D features generated from images~\cite{yao2018mvsnet,im2019dpsnet,wang2021patchmatchnet,duzceker2021deepvideomvs}. Then the depth map of the reference image can be regressed from the cost volume through 2D convolutions~\cite{wang2018mvdepthnet, huang2018deepmvs, hou2019multi} or 3D convolutions~\cite{yao2018mvsnet,im2019dpsnet}.
%

Most of the methods that can be considered for real-time applications utilize 2D convolutions.
DeepMVS~\cite{huang2018deepmvs} exploits patch matching for plane-sweep volume generation, and incorporates both intra-volume and inter-volume feature aggregation across an arbitrary number of input images.
%
MVDepthNet~\cite{wang2018mvdepthnet} is an efficient network enabling real-time applications. It generates a cost volume directly from the warped image pixel values, and regresses the depth via a lightweight encoder-decoder network composed of 2D convolutions and skip connections.
%
GPMVS~\cite{hou2019multi} further extends MVDepthNet with the introduction of Gaussian Process (GP) prior to the bottleneck layer. 
The intuition is to leverage a pose kernel to measure the difference between camera poses, and to encourage similar poses to have similar latent variables in the bottleneck layer. With only a slight computation increment originating from the GP prior constraint, GPMVS can achieve much higher accuracy on dense depth regression over MVDepthNet.
%
SimpleRecon~\cite{sayed2022simplerecon} achieves high accuracy for depth prediction by including extra information in the cost volume via parallel MLP reduction of readily-available metadata~-- such as dot product of features across multiple views, back-projected rays from pixels, pose distances, and a validity mask~-- but incurs a higher computational cost than competing methods.
%
In order to lift the 2D depth images into a 3D volumetric representation, traditional TSDF fusion~\cite{curless1996volumetric, newcombe2011kinectfusion} is typically utilized by these methods.
%
% that is useful for downstream tasks, 

%
MVSNet~\cite{yao2018mvsnet} %and DPSNet~\cite{im2019dpsnet} 
constructs a 3D cost volume based on the variance of deep features, and further regularizes and regresses the depth map of the reference image via 3D convolutions -- which enables higher accuracy than 2D convolutions but pays the cost of higher computation and memory consumption.
%
To alleviate this issue, and allow depth prediction at higher resolutions, Gu et al. propose a cascade 3D cost volume~\cite{gu2020cascade} -- narrowing the depth range of cost volume gradually from coarse to fine scales.
%
PatchmatchNet~\cite{wang2021patchmatchnet} imitates the traditional PatchMatch method~\cite{barnes2009patchmatch} by an end-to-end trainable architecture, which reduces the number of 3D convolutions needed in cost volume regularization and allows prediction at an even higher resolution than the cascade method~\cite{gu2020cascade}.
While the accuracy and efficiency of the MVS methods utilizing 3D convolutions is ever increasing,
they are still mostly amenable to offline processing.
%
%In this work, we opt to leverage GPMVS~\cite{hou2019multi} due to its overall reliability and efficiency, and augment this network with an additional uncertainty head to fit our needs. 



%
%DeepVideoMVS~\cite{duzceker2021deepvideomvs} applies a ConvLSTM cell~\cite{shi2015convolutional} on the bottleneck of encoder-decoder architecture for cost volume regularizations.  The ConvLSTM cell acts like a fusion module to account for the spatio-temporal relations between successive images in a video stream. 
%


%Distinct from cost volume based methods, there are also some works exploiting the point cloud learning for MVS.
%
%Chen et al. proposes a point-based framework~\cite{chen2019point}, which firstly predict a rough depth map and back-project it for generating 3D point cloud. In order to refine the previous depth map, they iteratviely predict depth residual from the point cloud assigned with aggregated image features.
%
%DELTAS~\cite{sinha2020deltas} detects and matches points of interest to recover a sparse point cloud by triangulation, and further densifies it to generate a dense depth map using convolutions. 
%
%3DVNet~\cite{rich20213dvnet} combines the MVS depth prediction method and volumetric feature volume based scene prediction methods.
%PointFlow algorithm [2]
%uses a volumetric 3D convolutional neural network (CNN) that operates in world space on all depth maps jointly. our 3D CNN operates on a feature augmented point cloud, allowing for effective aggregation of multi-view information and flexible iterative refinement of
%depth maps.
%%
%\noindent\textbf{Temporal Depth Fusion.}


% Volume based reconstruction
%\noindent\textbf
\subsection{Feature Volume-Based Scene Reconstruction.}
SurfaceNet~\cite{ji2017surfacenet} is among the first works to directly predict surface probability from 3D voxelized colored volumes from two image views using a 3D convolutional network. For generating the 3D voxelized colored volume, all the pixels on images are projected into 3D through the known camera intrinsics and extrinsics. Two colored volumes are then concatenated along the color channel, and regularized by 3D convolutions.
%
Atlas~\cite{murez2020atlas} extends this idea by replacing the colored volume with more informative deep feature volumes, and further enables an arbitrary number of multi-view images. Constructed 3D volumetric deep feature volumes across multiple views go through average pooling before being fed into the 3D convolutions.
%
TransformerFusion~\cite{murez2020atlas} and Vortx~\cite{stier2021vortx} exploit transformer-based attention mechanism for aggregating features from multiple image views instead of average pooling. TransformerFusion~\cite{murez2020atlas} also leverages the predicted attention weights to select the most relevant information for fusion.
In order to alleviate the effects of occlusion in the aggregation of multi-view image features, Vortx~\cite{stier2021vortx} predicts the projective occupancy probabilities, which are used as weights to produce the aggregated feature in the volume.
%


Note that none of the aforementioned feature volume-based methods are aiming for real-time applications. 
%
TransformerFusion~\cite{murez2020atlas} processes every image frame one by one, and gradually selects a certain number of the most relevant feature measurements for every voxel grid based on attention weights. Besides, expensive dense 3D convolutions are utilized to deal with the feature volume. Those mentioned assignment choices make TransformerFusion far from real-time \rev{capable}.
%
Vortx~\cite{stier2021vortx} does not work in an incremental way, and it predicts the TSDF map from the final integrated feature volume with the aggregated features from certain selected image views in the whole video stream. 
%

In contrast to the above methods, we focus on real-time incremental reconstruction based on feature \rev{volumes}.
The closest work to our method is NeuralRecon~\cite{sun2021neuralrecon}, which is also a baseline of our method. It performs feature volume-based reconstruction fragment by fragment at the first phase, which appears similar in spirit to active sliding windows in traditional SLAM methods~\cite{mourikis2007multi, %sibley2008sliding,
leutenegger2013keyframe, engel2017direct, zuo2019lic, %usenko2019visual
}. In order to get a globally consistent reconstruction, NeuralRecon further adopts GRU-Fusion at the second phase to fuse the fragment feature volumes over time, which can be regarded as an alternative to the conventional TSDF fusion~\cite{curless1996volumetric, newcombe2011kinectfusion}. 
%NeuralRecon is a real-time method, which incrementally constructs feature volumes and temporally fuse them to the global one.  
NeuralRecon does not have access to pick out the most relevant features from the whole video before the feature volume fusion and processing, thus it is supposed to have inferior performance than the full-batch methods~\cite{murez2020atlas,stier2021vortx}. %-- which have access to all images in the video sequence before making predictions.
%
Distinct from all the existing feature volume-based  methods that unproject and allocate features into the voxel grids along the whole rays in feature volume, we leverage MVS for rough dense depth predictions -- which allows us to allocate features to sparse voxels around the physical surfaces only. The retained sparsity keeps the memory consumption low and further enables high-resolution feature volume for scene reconstruction.
%



==> sections_main/03_methodology.tex <==
%!TEX root = ../main.tex

\section{Methodology}\label{sec:methodology}
%Our method utilizes depth priors to improve real-time incremental dense reconstruction based on feature volumes~\cite{sun2021neuralrecon,}. Here we describe our proposed incremental reconstruction method in detail.

%\subsection{Overview}
% NOTE: (nmerrill) I like this "sequence builder" notation: 
% https://math.stackexchange.com/questions/4352122/sequence-builder-notation
% \{.\} implies an unordered set
We take as input a fragment sequence of $N$ keyframe images $\{\bI_k\}_{k=0}^{N-1}$ along with their corresponding poses $\{ \bT_k\}_{k=0}^{N-1}$ and camera intrinsics $\{\bK_k\}_{k=0}^{N-1}$, $N=9$ is used in our work. Following~\cite{duzceker2021deepvideomvs, sun2021neuralrecon,}, we utilize a 2D feature extraction network composed of an MnasNet encoder~\cite{tan2019mnasnet} and feature pyramid network (FPN)~\cite{lin2017feature} style decoder. %  for increasing receptive filed and fetching features at multi levels 
%A fragment sequences consists of $N=9$ images in our training and testing stages.
% As in ~\cite{sun2021neuralrecon}, 
We unproject extracted features into a 3D aggregated feature volume representation and directly regress the sparse TSDF values from \rev{the} feature volume. The key insight in our method
is the use of {\em depth priors} to construct a feature volume that is sparse from the very start~--
%rather than allocating a dense feature volume and sparsifying later on as in~\cite{sun2021neuralrecon,}.
allowing our 3D network to focus on the surface from the very beginning without wasting effort in allocating and processing dense volumes.
%-- yielding more complete reconstructions and better accuracy in many cases.
An overview of our system can be seen in Fig.~\ref{fig:framework}.



%We directly regress the Truncated Signed Distance Value (TSDF) from the feature volume chunk. In order to efficiently and  sparsely allocate image features into the 3D volumetric chunk, we leverage a Multi-view Stereo (MVS) network to predict the rough depth maps and accompanying depth uncertainty maps, and precisely allocate features around the surface region recovered from predicted depth maps and bounded by uncertainty maps. At the training stage, we supervise the TSDF regression by ground-truth TSDF values, and supervise the MVS depth prediction by ground-truth depth maps $\{\bD_i\}$ corresponding to input images, while the depth uncertainty prediction is un-supervised. 

%
%In order to aggregate features across multiple views at each voxel location, we exploit self-attention~\cite{vaswani2017attention,stier2021vortx} for data-dependent aggregation.
%
%We incrementally build up the feature volume chunk by chunk, and fuse feature volume inside the chunk in to a global feature volume by GRU (Gated Recurrent Unit) ~\cite{chung2014empirical} fusion, following NeuralRecon~\cite{sun2021neuralrecon}. The GRU fusion~\cite{chung2014empirical}, which can be regarded as an data-driven alternative to temporally fuse features encoding TSDF values, and replace the linear fusion of TSDF values in conventional TSDF fusion. 
%
%Notably, before GRU fusion, we also augment the features with channels of TSDF value and weight calculated from conventional TSDF fusion of the predicted dense depth, which also provides valuable guidance for the neural network.
%
%We can predict TSDF values from the feature volume directly via a simple MLP later. As a common practice, marching cube method~\cite{lorensen1987marching} is leveraged to recover the final 3D surface mesh from the predicted TSDF values.
 

\subsection{MVS-Guided Sparse Feature Allocation}
Unlike existing feature volume-based methods~\cite{murez2020atlas, sun2021neuralrecon, stier2021vortx} that allocate dense feature volumes from unprojected features,
we utilize depth priors (depth map and its uncertainty) to allocate feature volume locations only where the physical surface is likely located. 
To get the depth priors of every keyframe in the fragment for efficient feature allocation, 
%and prevent from casting a ray and allocating features to all the voxels densely along the ray , 
we leverage GPMVS~\cite{hou2019multi} due to its appealing efficiency and adequate accuracy. Due to the modularity of our design, other MVS methods like~\cite{duzceker2021deepvideomvs, sayed2022simplerecon} could also be applied to our method.

\subsubsection{MVS-Based Depth and Uncertainty Prediction}\label{subsec:mvs}
%The original GPMVS firstly construct a cost volume for a pair of two images (consisting of one reference image and one source image), and apply a 2D encoder-decoder pipeline on the cost volume to predict dense depth for the reference image. To leverage the prior knowledge temporally about the relative camera pose between two images, a non-parametric Gaussian process prior is enforced at the bottleneck of the encoder-decoder streamline to encourage the model to generate similar latent embeddings for the pair of images with similar relative poses. GPMVS can take more than two keyframes as input. Follow the default training of GPMVS, we input three neighbor keyframes $\{\bI_0, \bI_1, \bI_2\}$ into GPMVS, and predict the depth of the reference frame in image pairs, $\{\bI_0, \bI_1\}, \{\bI_1, \bI_2\}, \{\bI_2, \bI_1\}$ (the first frame in every pair is regarded as reference frame). Just recall that a fragment of keyframes consists of 9 keyframes, we uniformly split the fragment sequence into three subsequences and each subsequence is comprised of 3 keyframes. Actually, three subsequences inside a fragment of neighboring keyframes are usually with similar appearance, and training by performing back-propagation with all the three subsequence at once can lead to overfitting of the model. In practice, we randomly select one from the three subsequences for training to alleviate the overfitting issue.

%
GPMVS~\cite{hou2019multi} predicts the inverse depth map $\hat{\bD}_{L_i}^{-1}$ at four scales $i \in \{0, 1, 2, 3\}$, and applies supervision at the four levels by resizing the ground truth inverse depth $\bD_{L_i}^{-1}$. Note that we use $\;\hat{\cdot}\;$ to denote the estimated/predicted variables and, for ease of notation, assume operations (inverse, $\exp$, etc.) to be element-wise throughout this paper. 
We augment the GPMVS network architecture to enable the prediction of dense depth uncertainty $\hat{\bB}$ which is parameterized by $\hat{\bB} = \exp(\hat{\bB}_{\mathrm{log}})$ to ensure a positive uncertainty value. To predict $\hat{\bB}_{\mathrm{log}}$ we simply duplicate the last three layers of the decoder in GPMVS to create a shallow second decoder head at the highest resolution.
%
%The three layers for variance prediction include a Conv layer, a Up-Conv layer (up-sample followed by Conv) and a final Conv layer predicting the final uncertainty. Input channels for the three levels are $128, 65, 64$, respectively.
%
For the highest GPMVS resolution $L_0$, following~\cite{bloesch2018codeslam, zuo2021codevio}, we apply the Laplacian maximum likelihood estimator (MLE) loss to enforce that the predicted uncertainty tightly bounds the true prediction error:
%
%\begin{align}
%	\label{eq:loss_mv}
%	\scalemath{.9}{
%		L_{\mathrm{mvs}} = 
%		\frac{|\hat{\bD}_{L_0}^{-1} - \bD_{L_0}^{-1}|
%		}{\hat{\bB}} + \log{\hat{\bB}} + \sum_{x=1}^{3} {|\hat{\bD}_{L_x}^{-1} - \bD_{L_x}^{-1}|}  
%	}
%\end{align}
%
\begin{align}
	\label{eq:loss_mv}
	%\scalemath{.9}{
 		\mathcal{L}^{(0)}_{\mathrm{mvs}} =
        \frac{1}{|\Omega|}
        \sum_{\bu \in \Omega}
        \frac{|\hat{D}_{L_0}^{-1}(\bu) - D_{L_0}^{-1}(\bu)|}{\hat{B}(\bu)} 
        + \log{\hat{B}(\bu)}
	%}
\end{align}
where $\Omega$ is the set of pixels with valid ground truth.
For the other three resolutions with no uncertainty prediction, we use the standard $\ell_1$ loss. The losses $\mathcal{L}^{(i)}_{\mathrm{mvs}}$ from all resolutions are added together with equal weights, and mean reduction is used across batches.
%
% We will assume that the depth is for the highest resolution and omit the subscript ${L_0}$ for the remainder of this paper.
%
For the remainder of this work, we will only use the (inverse) depth at the highest resolution, ${L_0}$, and omit the respective subscript for brevity.

We leverage linear uncertainty propagation to convert the uncertainty of inverse depth to the uncertainty of depth:
\begin{align}
	\hat{\bC} = \hat{\bD}^{2} \odot \hat{\bB}
\end{align}
\rev{where $\odot$ is the element-wise product.}
%Fig.~\ref{fig:depthuncer} exemplifies the predicted depth and uncertainty, and it can be found that the uncertainty map bounds the error of the predicted depth. 
%


% \begin{figure} [thb]
% 	\centering % trim={<left> <lower> <right> <upper>}
% 	\includegraphics[trim={0 0 0 2pt},clip,width=\columnwidth]{%
% 		figures/depthuncer_scannettest/scene0770_00_id343.jpg}
% 	\includegraphics[trim={0 0 0 2pt},clip,width=\columnwidth]{%
% 		figures/depthuncer_scannettest/scene0774_00_id307.jpg}
% 	\includegraphics[trim={0 0 0 2pt},clip,width=\columnwidth]{%
% 		figures/depthuncer_scannettest/scene0806_00_id64.jpg}
% 	\caption{ Some qualitative results on Scannet test split.
% 		It is formatted in columns of image, ground-truth depth (within 3 meters), followed by prediction, error, and predicted uncertainty of depth map.}
% 	\label{fig:depthuncer}
% % \vspace{-2em}
% \end{figure}


% \subsubsection{Surface Probability}
% Based on the predicted depth $\hat{\bD}$ following a Laplace distribution and the accompanying uncertainty $\hat{\bC}$, we are allowed to calculate the probability of being the surface with zero TSDF value for every individual voxel in the feature volume. Before calculating the surface probability, we need to convert predicted depth to range. For a pixel $[u, v, 1] $ with predicted depth value $\hat{\bD}$, and accompanying uncertainty $\hat{c}$, the range value $r$ of its corresponding 3D point is with mean $\hat{r}$ and uncertainty $\hat{v}$:
% \begin{align}
% &~	\hat{r} = \hat{\bD}*\sqrt{u^2+v^2+1}, \;\;\; \hat{v} = \frac{\hat{r}}{\hat{\bD}}*\hat{c} \notag \\
% &~	p(r|\hat{r}, \hat{v}) = \frac{1}{2 \hat{v}} \exp{(-\frac{r - \hat{r}}{\hat{v}})}
% \end{align}
% %
% where $p(r|\hat{r}, \hat{v}) $ is the surface probability density function under Laplace distribution along the range $r$. For a voxel with size $w$ and at range $r$ along the ray cast from the pixel $[u, v, 1]$, we can compute the probability of surface locating in that voxel by:
% \begin{align}
% \label{eq:surfprob}	
% p_{surf} \simeq  \int_{-\infty}^{r+w/2} p(r|\hat{r}, \hat{v})  \,dr - \int_{-\infty}^{r-w/2} p(r|\hat{r}, \hat{v})  \,dr 
% \end{align}
% %
% where the cumulative distribution function can be analytically computed:
% \begin{align}
% \scalemath{.85}{
% 	\int_{-\infty}^{r} p(r|\hat{r}, \hat{v})  \,dr = 0.5 + 0.5*{\rm{sign}}(r - \hat{r})\left( 1- \exp{\left( -\frac{|r - \hat{r}|}{\hat{v}}\right)} \right)
% }	
% \end{align}
% In Eq.~\eqref{eq:surfprob}, we assume the ray vertically penetrating the 3D voxel surfaces, which is not exactly true but a simple yet reasonable approximation.

% \begin{figure} [!t]
% 	\centering
% 	\includegraphics[width=\columnwidth]{%height=0.5\columnwidth
% 		figures/surface_prob}
% 	\caption{
% 	Illustration of surface probability along the range of the ray. 
% 	}
% 	\label{fig:surfaceprob}
% 	\vspace*{-2em}
% \end{figure}

\subsubsection{Sparse Feature Allocation}\label{subsec:feat_allocation}

\begin{figure} [!bth]
	\centering
	\includegraphics[width=0.8\columnwidth]{%
		figures/sparse_allocation1}
	\caption{
		2D illustration of sparse feature allocation with the predicted depth map $\hat{\bD}$ and accompanying uncertainty map $\hat{\bC}$.
	}
	\label{fig:sparseallocation}
	\vspace*{-.4em}
\end{figure}

%We carefully budget the feature volume allocation and try to make the voxels with allocated features as sparse as possible.  The sparser voxels mean less computation and less memory consumption in  subsequent 3D sparse convolutions and GRU fusion, which benefits the feature volume based method a lot.
Here we present the scheme to do sparse feature allocation based on casting the predicted depth and uncertainty (Sec.~\ref{subsec:mvs}) into sparse voxels.
%
Fig. \ref{fig:sparseallocation} shows a visual representation of how the sparse feature volume is constructed.
%
For each keyframe in a fragment, we utilize the predicted depth $\hat{\bD}$ and uncertainty map $\hat{\bC}$ to determine where we should allocate voxels in the sparse feature volume. 
%we firstly create a set of $2n+1$ depth hypotheses $\{ \hat{\bD}-n\bDelta, \cdots, \hat{\bD}-\bDelta, \hat{\bD}, \hat{\bD}+\bDelta, \cdots, \hat{\bD}+n\bDelta\}$, where the depth interval $\bDelta$ is the value of voxel size, and $n$ is calculated from the . For an individual depth primitive, we will check the validity of its every component pixels. 
Specifically, we only allocate voxels in the feature volume that lie along the ray of a pixel with positive predicted depth value and within the range of uncertainty bounds $[\hat{\bD}- s \hat{\bC}, \hat{\bD}+ s \hat{\bC}]$.
In our experiments, we use $s=2$.

%We generating 3D point clouds by back projecting all the valid pixels on all the depth primitives into 3D space. 
%
%Inside the fragment chunk, voxels where the back-projected points located are selected as valid voxels, and will be allocated image features into by projecting into image planes and fetching corresponding features across different keyframe views.



\subsection{Multi-view Feature Aggregation via Self Attention}
Deep image features at three resolutions are obtained by the feature extraction backbone, consisting of an efficient variant of \rev{MnasNet} encoder~\cite{tan2019mnasnet} followed by a feature pyramid network (FPN)~\cite{lin2017feature}. % to increase the receptive field of the extracted feature maps.
A 3D voxel location can be observed by multiple images from different viewpoints. We perform the feature aggregations in a content-aware way via multi-head self-attention~\cite{vaswani2017attention} at three scales. We first project a 3D voxel location into image planes across different views by the known camera poses and camera intrinsics, and fetch features for this specific voxel from the extracted multiple-scale feature maps through differentiable bilinear interpolation. Since the feature aggregations procedure at different scales is the same, we exemplify it at one scale. The fetched features from $N$ views, $\bF_{\mathrm{bp}} \in \mathbb{R}^{N \times C}$, with zero padding for the invisible views, and visibility binary mask $\bM \in \mathbb{R}^{N}$ are the input to the self-attention based feature aggregation module, which outputs the content-aware features with viewpoint and data dependencies:
%
\begin{align}
\bF_{\mathrm{attn}} = f_{\mathrm{attn}}(\bF_{\mathrm{bp}}, \bM_{\mathrm{attn}})
\end{align}
%
where the output feature $\bF_{\mathrm{attn}} \in \mathbb{R}^{N \times C}$ has the same feature channel with the input.
Following~\cite{stier2021vortx}, we realize the above self-attention aggregation module $f_{\mathrm{attn}}(\cdot)$ by two transformer layers following the original transformer pipeline~\cite{vaswani2017attention}. Each layer includes a multi-head attention mechanism (\rev{two heads in our implementation}), as well as layer normalization, linear layers with ReLU activation, and residual connections. All the query, key, and value features originate from the same input features in the multi-head attention mechanism. In practice, we use two heads for the multi-head attention module. The aggregated features $\bF_{\mathrm{attn}}$ are simply averaged to generate a single feature vector $\bF$  for the specific voxel.

\subsection{Fragment Reconstruction from Sparse Feature Volume}
% After allocating features across different views into sparse voxels, we leverage the self-attention mechanism in Transformer~\cite{vaswani2017attention} to process the raw image features for fusion, which shares the same spirit as ~\cite{stier2021vortx}. The self-attention module consists of 2 layers and is with 2 heads each layer.
% After the self-attended feature aggregation, we simply fuse the features across different views by average pooling.
\rev{After aggregating features from different views, we obtain a single feature vector within each non-empty voxel. We then directly regress the TSDF value of the voxel from this feature vector. }
With the predicted dense depth maps of keyframes in the fragment, it is handy to perform conventional TSDF-fusion~\cite{newcombe2011kinectfusion} and get the TSDF values and weights for every voxel inside the chunk. The TSDF value and weight are concatenated with the averaged image feature for subsequent 3D sparse convolutions~\cite{tang2020searching}. The final TSDF values of the chunk can be directly predicted from the feature volume by an MLP layer.

\subsection{Fragment to Global Fusion}
We follow NeuralRecon~\cite{sun2021neuralrecon} to fuse the fragment feature volume  into a global feature volume incrementally via GRU fusion~\cite{chung2014empirical}.
%which can be regarded as a data-driven alternative to temporally fuse features encoding  TSDF values, and replace the linear fusion of TSDF values in conventional TSDF fusion. 
For a feature vector $\bF_t$ originating from current fragment in the feature volume at time instant $t$, we fuse it with the historical feature $\bH_{t-1}$ at the same voxel location by GRU fusion. 
We observe that the volume resulting from traditional TSDF fusion with the predicted MVS depth is an additional useful feature for the network predicting the TSDF volume.
Thus, the fused TSDF values and weights, $\mathbf{S}_t$ and $\mathbf{S}_{Wt}$, from fusing the MVS depths are concatenated with features in order to guide the fusion process. After the concatenation with increased feature dimensions, we leverage single-layer MLPs for feature dimension reduction.%\note{Also talk about the augmentation of TSDF and weights.}
\begin{subequations}
	\begin{align}
		\mathbf{H}'_{t-1} &= \operatorname{MLP}_H\left(\left[\mathbf{H}_{t-1}, \mathbf{S}_t, \mathbf{S}_{Wt}\right]\right)\\
		\mathbf{F}'_{t} &= \operatorname{MLP}_F\left(\left[\mathbf{F}_{t}, \mathbf{S}_t, \mathbf{S}_{Wt}\right]\right)\\
		\bz_t &=\operatorname{sigmoid}\left(\operatorname{SpConv}\left(\left[\mathbf{H}'_{t-1}, \mathbf{F}'_t\right]\right)\right) \\
		\br_t &=\operatorname{sigmoid}\left(\operatorname{SpConv}\left(\left[\mathbf{H}'_{t-1}, \mathbf{F}'_t\right]\right)\right) \\
		\breve{\mathbf{H}}_t &=\tanh \left(\operatorname{SpConv}\left(\left[\br_t \odot \mathbf{H}'_{t-1}, \mathbf{F}'_t\right]\right)\right) \\
		\mathbf{H}_t &=\left(\mathbf{I}-\bz_t\right) \odot \mathbf{H}'_{t-1}+\bz_t \odot \breve{\mathbf{H}}_t
	\end{align}
\end{subequations}
where $\bz_t$ is the update gate vector, $\br_t$ the reset gate vector, $\left[ \cdot, \cdot \right]$ the concatenation operator. $\operatorname{SpConv}$ denotes the sparse point-voxel convolution operation~\cite{tang2020searching}. With the above GRU fusion, we can temporally fuse features and keep updating the visible feature volumes at three scales.

\subsection{Implementation Details}
We maintain three levels of feature volumes and regress the TSDF values $\bS_{L_i}$ from them in a coarse to fine manner. In order to further sparsify the feature volume for the proceeding scales, we also predict occupancy values $\bO_{L_x}$ from feature volumes at all scales with simple MLP layers. If the occupancy prediction of a voxel at a coarser scale is lower than a threshold (0.5), that voxel is redeemed as empty and will not be involved in feature allocation and prediction at finer scales~\cite{sun2021neuralrecon}. 
Overall, the training loss for regressing TSDF and occupancy at a single resolution $i$ is:
\begin{align}
	\label{eq:loss_recon}
	%\scalemath{.9}{
	\mathcal{L}_{\mathrm{recon}}^{(i)} =
     \frac{1}{|\Lambda|}
    \sum_{\bx \in \Lambda}
    \bigg(  & \lambda_1  {|{\rm{logt}}(\hat{S}_{L_i}(\bx)) 
    - {\rm{logt}}({S}_{L_i}(\bx))|}  \bigg. \notag \\
    \bigg. & + \lambda_2 {\rm{BCE}}({\hat{O}_{L_i}(\bx), O_{L_i}(\bx)})  \bigg)
     %}
\end{align}
where $\Lambda$ is the set of voxels with valid ground truth, and ${\rm{logt}}(\bS_{L_i}) = {\rm{sign}}(\bS_{L_i})\log(|\bS_{L_i} + 1|)$ denotes the log-transform~\cite{sun2021neuralrecon,dai2020sg}, and $\rm{BCE}$ denotes the binary cross-entropy (BCE) loss.
\rev{We have $\lambda_1 = \lambda_2$ for balancing the two loss terms in our training.}
We add the losses $\mathcal{L}_{\mathrm{recon}}^{(i)} $ at each scale and apply mean reduction over batches.
%

% with equal weighting 
% It is worthwhile to mention that we only account for the loss in observed voxels like~\cite{dai2020sg}, in order to alleviate the issue of incomplete ground-truth TSDF and occupancy. In this paper, observed voxels denotes the ones between the camera origin and outward uncertainty boundary in Fig.~\ref{fig:sparseallocation}.
%

The input images are at resolution $640\times480$, while the features at three levels are fetched from feature maps at resolutions $320\times240$, $160\times120$, $80\times60$ with channels $24, 40, 80$, respectively.
GPMVS requires input images with resolution $320 \times 256$, which are obtained by bilinear interpolation-based downsampling. Dense depth maps are downsampled via nearest neighbor to better preserve sharp edges. We utilize the TorchSparse~\cite{tang2020searching} implementation of sparse 3D convolutions in our method.



 





==> sections_main/04_experiment.tex <==
%!TEX root = ../main.tex
\section{Experiments}\label{sec:exp}

\begin{table}[!t]
%	\vspace{-1.2cm}
	\centering % Comp (dist2), Acc (dist1)
	\caption{3D geometry metrics evaluated on ScanNet test split. 
		Note that the methods under the middle line are feature-volume-based incremental reconstruction methods, while the others are not.}
	\label{tab:scannet-3d}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{cccccc}
			\Xhline{3\arrayrulewidth}
			Method       & Comp $\downarrow$ & Acc $\downarrow$   & Recall $\uparrow$ & Prec $\uparrow$   & F-score  $\uparrow$   \\ \hline
			COLMAP \cite{schonberger2016pixelwise} & 0.069   & 0.135   & 0.634   & 0.505   & 0.558 \\ 
			MVDepthNet \cite{wang2018mvdepthnet}     &  \textbf{0.040}   & 0.240   & 0.831   & 0.208   & 0.329    \\ 
			DPSNet \cite{im2019dpsnet} & {0.045}   & 0.284   & \textbf{0.793}   & 0.223   & 0.344  \\
			%% GPMVS \cite{hou2019multi} & \textbf{0.031}  & 0.879   & \textbf{0.871}  & 0.188   & 0.304      \\ 
			GPMVS \cite{hou2019multi} & 0.105  & 0.191   & 0.423  & 0.339   & 0.373     \\ 
			Atlas \cite{murez2020atlas} & 0.083  & 0.101   & 0.566 & 0.600   & 0.579  \\ 
			Vortx \cite{stier2021vortx} & 0.081 & \textbf{0.062} & 0.605 & \textbf{0.689} & \textbf{0.643} \\
			\hline
			\rowcolor[gray]{0.902}
			NeuralRecon \cite{sun2021neuralrecon} & 0.137   & \textbf{0.056}  & 0.470   & \textbf{0.678}  & 0.553 \\
			\rowcolor[gray]{0.902}
			Ours & \textbf{0.110} & 0.058 & 0.505 & 0.665 & 0.572 \\
   			\rowcolor[gray]{0.902}
                \rev{Ours (High Reso)} & 0.116 & \textbf{0.056} & \textbf{ 0.525} & 0.675 & \textbf{0.589} \\
			% \rev{Ours (High Reso)} & \textbf{0.103} & 0.063 & \textbf{ 0.538} & 0.658 & \textbf{0.590} \\
			% \rowcolor[gray]{0.902}
			% %% SingleLayerTrimResolution0.02 \rev{Ours (High Reso +)} & \textbf{0.098} & 0.061 &\textbf{ 0.552} & 0.666 & \textbf{0.602}  \\
			\Xhline{3\arrayrulewidth}
		\end{tabular}
	}
\end{table}

\begin{table}[!t]
	\centering
	\caption{2D depth metrics evaluated on ScanNet test split. Note that the methods under the middle line are feature-volume-based incremental reconstruction methods, while the others are not.}	
	\label{tab:scannet-2d}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{ccccccccc}
			\Xhline{3\arrayrulewidth}
			Method                                        & Abs-rel $\downarrow$ & Abs-diff $\downarrow$ & Sq-rel $\downarrow$ & RMSE $\downarrow$ & $\delta < 1.25$ $\uparrow$& Comp $\uparrow$ \\ \hline
			COLMAP \cite{schonberger2016pixelwise}                                        & 0.137          & 0.264          & 0.138          & 0.502          & 83.4                    & 0.871           \\ 
			MVDepthNet \cite{wang2018mvdepthnet}                                   & 0.098          & 0.191          & 0.061          & 0.293          & 89.6                    & 0.928           \\ 
			DPSNet \cite{im2019dpsnet}                                       & 0.087          & 0.158          & \textbf{0.035}          & 0.232          & 92.5           & 0.928           \\ 
			% GPMVS (altas paper) \cite{hou2019multi}                                        & 0.130          & 0.239          & 0.339          & 0.472          & 90.6                    & 0.928           \\
			GPMVS \cite{hou2019multi}  &   0.088 &  0.206 & 0.053 & 0.359 & 90.3 & 0.928     \\ 
			% GPMVS-rend  \cite{hou2019multi} & 0.113 & 0.187 & 0.082 & 0.323 & 87.3 & 0.976      \\
			Atlas \cite{murez2020atlas}    & 0.065          &
			0.123          & 0.045          & 0.249          & 92.4                    & \textbf{0.986}  \\
			Vortx \cite{stier2021vortx} & \textbf{0.057} & \textbf{0.090} & \textbf{0.035} & \textbf{0.197} & \textbf{93.9} & 0.951 \\ 
			\hline
			\rowcolor[gray]{0.902}
			NeuralRecon \cite{sun2021neuralrecon}                                       & 0.064 & 0.097 & 0.036 & 0.191 & 93.5           & 0.888           \\ 
			\rowcolor[gray]{0.902}
			ours & 0.057 & 0.092 & {0.030} & 0.183 & 94.2 & \textbf{0.913} \\
   			\rowcolor[gray]{0.902}
      \rev{ours (High Reso)} & \textbf{0.052} & \textbf{0.087} & \textbf{0.025} & \textbf{0.175} & \textbf{94.8}& 0.906 \\
			% \rev{ours (High Reso)} & \textbf{0.056} & 0.093& \textbf{0.029} & 0.186 & \textbf{94.3}& \textbf{0.920} \\
			% \rowcolor[gray]{0.902}
			% % %% SingleLayerTrimResolution0.02 \rev{ours (High Reso +)} & {0.057} & 0.094& {0.030} & 0.187 & \textbf{94.3}& {0.915} \\
			\Xhline{3\arrayrulewidth}
		\end{tabular}
	}
\end{table}


%\input{figures/meshes.tex}
\input{figures/meshes_wrect.tex}

\subsection{Datasets and Metrics}
For all the evaluations, we use the ScanNet dataset~\cite{dai2017scannet} for training, which consists of 1513 RGBD sequences collected in 707 indoor scenes. We follow the official training and test splits, which are 1201 and 100 sequences, respectively. Besides the ScanNet test split, we also test the ScanNet-trained network zero-shot on TUM-RGBD~\cite{sturm2012benchmark} (13 sequences following~\cite{stier2021vortx}), and our own collected dataset without any finetuning.
%
For 3D metrics, we evaluate the final reconstructed surface mesh extracted from the predicted TSDF volume against the officially provided mesh on ScanNet, and we generate our own meshes on TUM-RGBD and our own collected datasets through conventional TSDF fusion using the ground truth depth. \rev{Following the evaluation protocol~\cite{murez2020atlas, sun2021neuralrecon} exactly, we calculate 3D metrics, including accuracy, completeness, precision, recall, and F-score, across uniformly sampled points with a 2-centimeter resolution from dense meshes. For computing these 3D metrics, a distance threshold of 5 centimeters was used.} We regard the F-score to be the most representative metric to reflect the quality of 3D reconstruction, since it is involved with both precision and recall.
%
\rev{}
%
Regarding 2D metrics, we evaluate the rendered depth maps at all the image views for the feature volume-based scene reconstruction methods, against the provided raw depth maps with a truncation of 10 meters. The MVS methods predicting dense depth maps directly allow for handy evaluations.

\subsection{Training Details}

We use ScanNet dataset~\cite{dai2017scannet} for training. 
% which consists of 1513 RGBD sequences collected in 707 indoor scenarios. We follow the official training and test splits, which are 1201 and 100 sequences, respectively.
%
Ground truth TSDF volumes are generated from raw depth maps and given camera poses by conventional TSDF fusion~\cite{curless1996volumetric, newcombe2011kinectfusion}. Note that we discard all the depths over $3m$ like existing methods~\cite{sun2021neuralrecon, stier2021vortx}. %, due to the high measurement noises.
%
Before training the feature volume pipeline, we need to fine-tune the lightweight GPMVS~\cite{hou2019multi} depth prediction network for 12 epochs, then train the depth variance prediction network for 4 epochs from randomly initialized weights. Note that, GPMVS is frozen in subsequent training, while the weights of the variance network are kept updated. 
%
We have two phases for training the feature volume pipeline for incremental reconstruction from monocular videos.
At the first phase, we train the fragment-wise reconstruction network, regressing TSDF from feature volume for 20 epochs.
%
The network learns how to predict TSDF from aggregated features in a fragment volume with size $3.84m \times 3.84m \times 3.84 m$. Finally, we train the network at the second phase with the GRU fusion network together for 30 epochs. 
%
Adam optimizer with $\beta_1 = 0.9, \beta_2 = 0.999$ is adopted for training the networks, and the learning rate is $1e-3$ at the beginning and decreased by half at epochs $12, 24, 48$ in the two-phase training.
%
The finest voxel resolution is $4cm$ by default, and is reduced to $2cm$ for our high-resolution variant. The batch size is $32$ by default, and $8$ for the higher resolution variant.
%
% Finetue GPMS firstly （37epochs）, train the variance network(12epochs), train neucon with frozen GPMVS at two stages.

\subsection{Evaluation on ScanNet}
The evaluation results with both 3D metrics and 2D metrics are shown in Table~\ref{tab:scannet-3d} and Table~\ref{tab:scannet-2d}, respectively. We compare the proposed method, \textit{Ours}, with state-of-the-art traditional structure-from-motion method, COLMAP~\cite{schonberger2016pixelwise}, multi-view stereo networks including MVDepthNet~\cite{wang2018mvdepthnet}, DPSNet \cite{im2019dpsnet}, and GPMVS \cite{hou2019multi}, as well as all the open-source feature-volume-based methods including Atlas \cite{murez2020atlas},  Vortx \cite{stier2021vortx}, and NeuralRecon \cite{sun2021neuralrecon}.
%
Our method with high-resolution feature volume is named \textit{Ours (High Reso)}. It should be noted all the compared methods are evaluated with the same protocol.
%
% We are also willing to compare to TransformerFusion~\cite{murez2020atlas}, however it is not open-sourced yet at the submission time of this paper.
%
All compared deep-learning-based methods have been trained or fine-tuned on the ScanNet dataset. The results of  COLMAP, MVDepthNet, and DPSNet are taken from~\cite{murez2020atlas}, while GPMVS, Atlas, Vortx, and NeuralRecon are evaluated by ourselves.


The proposed incremental feature volume-based method outperforms the existing incremental method, NeuralRecon, regarding the representative 3D reconstruction metric -- the F-score. The advantages on F-score are mainly from the higher recall, while the proposed method and NeuralRecon have very similar precision. With the incorporation of MVS depth and depth uncertainty in our method, more structures can be recovered compared to the pure feature volume-based NeuralRecon.
%
When the voxel size of feature volume is decreased from $4cm$ to $2cm$, dubbed as \textit{Ours (High Reso)}, the overall quality of reconstruction can be further improved. 
%
We attempted to train NeuralRecon~\cite{sun2021neuralrecon} with a high-resolution feature volume as well for a direct comparison, but the training network was unable to fit in GPU memory (see Sec. \ref{subsec:memruntime}).
%
It should also be noted that both Atlas~\cite{murez2020atlas} and  Vortx~\cite{stier2021vortx} are offline methods, and have the access to full batch data with global context before predicting TSDF values from features, and they are expected to exhibit better performance than our real-time incremental method. Actually, \textit{Ours} as the real-time incremental method has very close performance to Atlas~\cite{murez2020atlas} and slightly better performance than traditional offline method COLMAP~\cite{schonberger2016pixelwise}. 
%

We also show qualitative results of the meshes generated from different methods in Fig.~\ref{fig:meshes}.
%where we denote the shown scenarios as scenario $1 - 9$ from top to bottom.
%
The MVS method, GPMVS~\cite{hou2019multi}, which is also leveraged in our pipeline to guide the feature allocation, suffers from significant artifacts. With the feature volume-based regularization and denoising, our method is able to remove the main artifacts in MVS reconstruction. This also verifies that the predicted depth and depth uncertainty for feature allocation only near the surface voxels are reasonable, and have provided the rough shape sufficient for the proceeding feature volume-based reconstruction.
%
It is found that \textit{Ours} and \textit{Ours (High Reso)} have the potential to recover more details about objects, such as the table leg, toilet, and chair. 
%
Atlas~\cite{murez2020atlas} and  Vortx~\cite{stier2021vortx} are prone to recover more complete walls and floors, but their predictions can be over-smoothed to miss details of objects, and over-filled with hallucinated structures.

\input{figures/tanktemple_mesh}


\subsection{Generalization on TUM-RGBD}
To examine the generalization of the proposed method, we also conduct comparisons on TUM-RGBD dataset~\cite{sturm2012benchmark}. We only compare to the incremental feature volume-based methods. We follow exactly the identical keyframing strategy as the one on Scannnet dataset. The 3D evaluation metrics are shown in Table~\ref{tab:tumrgbd}. We can find that \textit{Ours} outperforms NeuralRecon~\cite{sun2021neuralrecon}. Our high-resolution variant has obvious advantages over the default resolution. 

%\begin{table*}[tbh]
%	\centering % Comp (dist2), Acc (dist1)
%	\caption{Evaluated on TUM-RGBD dataset.}
%	\label{tab:tumrgbd}
%	\resizebox{\textwidth}{!}{
%		\begin{tabular}{cccccccccccc}
%			\Xhline{3\arrayrulewidth}
%			Method       & Comp $\downarrow$ & Acc $\downarrow$   & Recall $\uparrow$ & Prec $\uparrow$   & F-score  $\uparrow$  & Abs-rel $\downarrow$ & Abs-diff $\downarrow$ & Sq-rel $\downarrow$ & RMSE $\downarrow$ & $\delta < 1.25$ $\uparrow$& Comp $\uparrow$  \\ \hline
%
%			NeuralRecon \cite{sun2021neuralrecon} & 0.285   & 0.101 & 0.109& 0.391& 0.169& 0.083& 0.141& 0.060& 0.270& 93.9& 0.815  \\
%			Ours & 0.252 & 0.123 & 0.133 & 0.369 & 0.195 &  0.100 & 0.274& 0.108& 0.419& 87.4 & 0.870  \\
%			Ours (High Reso) & 0.192& 0.084& 0.199& 0.586& 0.295& 0.070& 0.171& 0.063& 0.279& 92.9& 0.819 \\
%			\Xhline{3\arrayrulewidth}
%		\end{tabular}
%	}
%\end{table*}

\begin{table}[tbh]
	\centering % Comp (dist2), Acc (dist1)
	\caption{Evaluated on TUM-RGBD dataset.}
	\label{tab:tumrgbd}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{cccccc}
			\Xhline{3\arrayrulewidth}
			Method       & Comp $\downarrow$ & Acc $\downarrow$   & Recall $\uparrow$ & Prec $\uparrow$   & F-score  $\uparrow$  \\ \hline
			\rowcolor[gray]{0.902}
			NeuralRecon \cite{sun2021neuralrecon} & 0.285   & 0.101 & 0.109& 0.391& 0.169  \\
			\rowcolor[gray]{0.902}
			Ours & 0.252 & 0.123 & 0.133 & 0.369 & 0.195  \\
			\rowcolor[gray]{0.902}
			\rev{Ours (High Reso)}& \textbf{0.192}& \textbf{0.084}& \textbf{0.199}& \textbf{0.586}& \textbf{0.295} \\
			\Xhline{3\arrayrulewidth}
		\end{tabular}
	}
 \vspace{-2em}
\end{table}



%\subsection{\color{blue}Generalization on Large-Scale Outdoor Tanks and Temples }
\subsection{Generalization on Tanks \& Temples }
\rev{We further conduct evaluations in two large-scale outdoor scenarios, ``Barn" and ``Courthouse", using the Tanks \& Temples dataset~\cite{tanktemple2017} without any fine-tuning of the network weights trained on the indoor ScanNet dataset~\cite{dai2017scannet}.
%
Our proposed method is designed to maintain sparsity in the feature volume, making it well-suited for large-scale volumetric reconstruction where most voxel grids are physically empty. In contrast, allocating features to a large number of voxels in dense volume can become computationally intractable. 
%
In order to run NeuralRecon~\cite{sun2021neuralrecon} successfully on these large-scale scenarios, the poses of images for all the compared methods are scaled down to be 5 to 10 times smaller.  
%The dense reconstruction results are qualitatively shown in Fig.~\ref{fig:meshes_tanktemple}.
%
 The dense reconstruction results are qualitatively depicted in Fig.~\ref{fig:meshes_tanktemple}. 
 Our method demonstrates strong generalization capabilities in outdoor large-scale scenarios, visibly outperforming NeuralRecon with much more desirable reconstruction results.  Moreover, our high-resolution reconstruction can recover finer details and more accurate scene structures.
}


\subsection{Generalization on Self-Collected Data}
\begin{figure*} [thb]
        \centering
	\newcommand{\w}{.20\textwidth}
	\centering % trim={<left> <lower> <right> <upper>}
	\begin{subfigure}[t]{\w}
		\caption*{\textbf{NeuralRecon~\cite{sun2021neuralrecon}}}
		\includegraphics[width=0.85\columnwidth]{
  % figures/showmesh_realsense/06-11-2022-16-54-28/snapshot00_L01.png
  figures/showmesh_realsense/06-11-2022-16-54-28/neucon02.png
  }
	\end{subfigure}
 \hspace{-7pt}
	\begin{subfigure}[t]{\w}
		\caption*{\textbf{Ours}}
		\includegraphics[width=0.85\columnwidth]{
  % figures/showmesh_realsense/06-11-2022-16-54-28/snapshot00_L02.png
  figures/showmesh_realsense/06-11-2022-16-54-28/ours04.png
   }
	\end{subfigure}
 \hspace{-7pt}
	\begin{subfigure}[t]{\w}
		\caption*{\textbf{Ours (High Reso)}}
		\includegraphics[width=0.85\columnwidth]{
  %figures/showmesh_realsense/06-11-2022-16-54-28/snapshot00_L03.png
  figures/showmesh_realsense/06-11-2022-16-54-28/ours_high03.png
  }
	\end{subfigure}
 \hspace{-7pt}
	\begin{subfigure}[t]{\w}
		\caption*{\textbf{GT}}
	\includegraphics[width=0.85\columnwidth]{
 %figures/showmesh_realsense/06-11-2022-16-54-28/snapshot00_L00.png
   figures/showmesh_realsense/06-11-2022-16-54-28/gt01.png
  }
	\end{subfigure}
 \hspace{-7pt}
	\begin{subfigure}[t]{\w}
	\caption*{\textbf{RGB}}	
	\includegraphics[width=0.85\columnwidth]{%
		figures/showmesh_realsense/1667750135092329472.png}
	\end{subfigure}%\hspace{-9pt}
	\caption{Qualitative results of a representative sequence from our self-collected dataset.} % It is formatted as image, ground-truth mesh, and followed by meshes coming from NeuralRecon~\cite{sun2021neuralrecon}, Ours, and Ours (Hight Reso).
	\label{fig:meshes_realsense}
    % \vspace{-1em}
\end{figure*}

We also collect our own dataset with 8 sequences in indoor scenarios by the Realsense D455 RGBD camera~\footnote{https://www.intelrealsense.com/depth-camera-d455}. We record the grayscale stereo images, RGB images, depth maps, and IMU data streamed from the camera.
The stereo images and IMU data are fed into a visual-inertial SLAM system, OKVIS 2.0~\cite{leutenegger2022okvis2}, for getting accurate 6DoF poses. 
%We further compute the poses at time instants of collecting synchronized depth and RGB pairs via interpolations. 
A snapshot of a typical scenario, and the reconstructed meshes from compared methods are shown in Fig.~\ref{fig:meshes_realsense}, where we can easily find that our methods can recover more geometric details than NeuralRecon~\cite{sun2021neuralrecon}. The quantitative 3D metric evaluations are also shown in Table~\ref{tab:realsense}.

%\begin{table*}[tbh]
%	\centering % Comp (dist2), Acc (dist1)
%	\caption{Evaluated on our own collected data.}
%	\label{tab:realsense}
%	\resizebox{\textwidth}{!}{
%		\begin{tabular}{cccccccccccc}
%			\Xhline{3\arrayrulewidth}
%			Method       & Comp $\downarrow$ & Acc $\downarrow$   & Recall $\uparrow$ & Prec $\uparrow$   & F-score  $\uparrow$  & Abs-rel $\downarrow$ & Abs-diff $\downarrow$ & Sq-rel $\downarrow$ & RMSE $\downarrow$ & $\delta < 1.25$ $\uparrow$& Comp $\uparrow$  \\ \hline
%			
%			NeuralRecon \cite{sun2021neuralrecon} & 0.203& 0.034& 0.214& 0.768& 0.334& 0.177& 0.283& 0.099& 0.396& 82.5& 0.948 \\
%			Ours & 0.145& 0.039& 0.257& 0.719& 0.379& 0.216& 0.341& 0.124& 0.439& 73.6& 98.4   \\
%			Ours (High Reso) & 0.139& 0.047& 0.280& 0.679& 0.396& 0.241& 0.382& 0.146& 0.480& 65.6& 96.8 \\
%			\Xhline{3\arrayrulewidth}
%		\end{tabular}
%	}
%\end{table*}

\begin{table}[tbh]
	\centering % Comp (dist2), Acc (dist1)
	\caption{Evaluated on our own collected data.}
	\label{tab:realsense}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{cccccc}
			\Xhline{3\arrayrulewidth}
			Method       & Comp $\downarrow$ & Acc $\downarrow$   & Recall $\uparrow$ & Prec $\uparrow$   & F-score  $\uparrow$   \\ \hline
			\rowcolor[gray]{0.902}
			NeuralRecon \cite{sun2021neuralrecon} & 0.205& \textbf{0.034}& 0.215& \textbf{0.774}& 0.335 \\
			\rowcolor[gray]{0.902}
			Ours & 0.144& 0.040& 0.255& 0.711& 0.374  \\
			\rowcolor[gray]{0.902}
			\rev{Ours (High Reso)} & \textbf{0.143}& 0.045& \textbf{0.268}& 0.683& \textbf{0.385} \\
			\Xhline{3\arrayrulewidth}
		\end{tabular}
	}
 \vspace{-2em}
\end{table}

\subsection{Memory and Runtime} \label{subsec:memruntime}
%
% The runtime evaluation is performed on a cluster with an RTX6000@24GB GPU and 4 Intel Xeon 6248 CPU Cores@2.5GHz allocated. % (NOTE: CHECH with quirin, whether it is 4 physical CPUs or cores)
%
We conducted runtime and memory evaluations of the inference stage on a desktop computer equipped with an RTX5000@16GB GPU and 8 Intel i7-11700k CPU Cores@3.6GHz. 
%
In Table~\ref{tab:mem_runtime}, we report the averaged time taken for MVS depth recovery, feature encoding, feature aggregation, TSDF-Fusion of MVS depths, 3D sparse CNN, GRU fusion, and the total processing time for a volume chunk with 9 keyframes. The experiment is conducted on a typical large-scale indoor sequence of ScanNet at the inference stage. %We excluded some time consumption related to data conversion and management. 
%The total time consumption and Keyframes per second reflect the overall efficiency of the methods.}
%  Note that all the methods involve three levels of pyramid feature volume. As a result, feature aggregation, 3D sparse CNN, and GRU fusion are each performed three times during a single forward pass.
%
Despite incorporating MVS depth and self-attention,
our method can run incremental reconstruction in real-time at 12.70 keyframes per second \rev{, with a slightly increased memory footprint compared to NeuralRecon.}
\rev{At the high resolution, our method runs at 5 keyframes per second.}
Although this is admittedly slower than NeuralRecon, which can run at 41 keyframes per second on the same device, it should be noted that our method is still real-time capable
since keyframes in a typical real-time SLAM system (e.g., \cite{leutenegger2022okvis2})
are created at a far lower frequency than the framerate. 
%

Our method is additionally highly memory-efficient in terms of voxel allocation.
%
At the inference stage, compared with the `dense' feature volume of NeuralRecon, the numbers of the non-empty voxel with allocated features in our sparse volume are significantly decreased by $67.71\%, 48.24\%, 30.71\%$  at three levels respectively.
% $74.61\%, 55.62\%, 34.29\%$
The feature volume in NeuralRecon is initially dense, and is sparsified by the network from coarse to fine levels.
This means that, in the initial phases of training, before the network learns to sparsify well, a nearly dense volume makes its way through the sparse 3D convolution network.
%
In our experiments, we did not train NeuralRecon at the high resolution due to this issue since the required GPU memory exceeded 42GB -- even with batch size 1.
In contrast, due to our MVS-guided sparse volume allocation, which makes feature volumes sparse at all three levels, we are able to train at the higher resolution even with the memory-intensive attention mechanism involved, consuming GPU memory around 28GB during training.
%



%We also disclose the memory consumption and runtime of the incremental-feature-volume methods on Scannet test split in Table~\ref{tab:mem_runtime}. The evaluation is performed on a cluster with a RTX6000@24GB GPU and 4 Intel Xeon 6248 CPUs@2.5GHz allocated. 
%
%We showcase the runtime of MVS depth inference, 2D CNN feature encoder, feature aggregation, 3D sparse CNN, GRU fusion and the total consuming time of processing a chunk with 9 keyframes. It can be seen that our method can run in real time around 7.96 keyframes/second. Compared with neural recon, we leverage the attention mechanism for feature aggregation, which leads to increment of runtime but better reconstruction result. 
%
%The numbers of nonempty voxels with allocated features at three levels are also counted. Compared with the dense feature volume of NeuralRecon, our valid voxels numbers for processing are significantly decreased $74.61\%, 55.62\%, 34.29\%$ at three levels respectively.
%
% The allocated memories of Pytorch for the inference of different methods are shown.  
%
%It should be noted that the memory consumption for training can be significantly higher than inference, as well as the number of nonempty voxels. 
%We struggle to train the NeuralRecon at high resolution, since it needs more than 32GB of GPU memory for a single batch. On the other hand, ours (high resolution) with the additional memory-intensive attention mechanism only needs around 28.9GB GPU memory to train -- benefiting from the MVS-guided sparse feature volume.
%
% For training NeuralRecon, Ours, and Ours (High Reso) with a single batch, Pytorch need to reserve 6.374GB, 10.43GB, and 28.90GB GPU memories, while training NeuralRecon with high resolution needs around 35.65GB memories.

\iffalse
\begin{table*}[tbh]
\color{blue}
	\centering % Comp (dist2), Acc (dist1)
	\caption{Mean of runtime(second), allocated memory(GB) and number of nonempty voxels in feature volumes on Scannet test split.}
	% Note the memory cosumption here is the allocated memeory. Actually, the reserved memeory are 2.021 (neuralrecon), 3.034 or 3.316 (ours),18.146(ours high)
	\label{tab:mem_runtime}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{cccccccC{0.5cm}cccc}\cmidrule[3\arrayrulewidth]{1-7}\cmidrule[3\arrayrulewidth]{9-12}
			Method       & MVS Dep. & Feat. Enc.  & Feat. Agg. & 3D SpCNN   & GRU Fusion & Total & & Voxels L0 & Voxels L1& Voxels L2 & Memory (GB)\\ \cline{1-7}\cline{9-12}
  	NeuralRecon \cite{sun2021neuralrecon} & - & 0.030& 0.028 & 0.035 & 0.023 & 0.299& &7267.57 &15954.09 &58328.85 & 0.200 \\
%			Ours & 0.323& 0.027& 0.035& 0.022& 0.019& 1.253& & 1560.19 & 7669.65& 41094.30&  0.538 \\
			Ours & 0.327& 0.027& 0.041& 0.024& 0.020& 1.130 & & 1844.11 &7080.08 & 38330.30& 0.546 \\
			Ours (High Reso) & 0.327& 0.027& 0.276& 0.086& 0.128& 3.978& & 10574.00& 58550.53& 334563.45& 1.704 \\
			\cmidrule[3\arrayrulewidth]{1-7}\cmidrule[3\arrayrulewidth]{9-12}
		\end{tabular}
	}
\end{table*}
\fi

\iffalse
\begin{table*}[tbh]
	\centering % Comp (dist2), Acc (dist1)
	\caption{\color{blue} Mean of runtime(Second) and memory consumption (GB) on a typical sequence of Scannet.}
	\label{tab:mem_runtime}
	\resizebox{0.85\textwidth}{!}{
	    \color{blue}
		\begin{tabular}{cccccccC{0.3cm}cc}\cmidrule[3\arrayrulewidth]{1-7}\cmidrule[3\arrayrulewidth]{9-10}
			Method       & MVS Dep. & Feat. Enc.  & Feat. Agg. & 3D SpCNN   & GRU Fusion & Total & &  Kf./Sec.& Memory (GB)\\ \cline{1-7}\cline{9-10}
  	        NeuralRecon \cite{sun2021neuralrecon} & - & 0.037& 0.004 & 0.032 & 0.021 & 0.219& & 39.30& 0.988 \\
			Ours & 0.375& 0.025& 0.033& 0.020& 0.019& 0.709 & &12.56 & 1.68 \\
			Ours (High Reso) & 0.386& 0.025& 0.191& 0.075& 0.106 & 1.786& &5.01& 9.06 \\
			\cmidrule[3\arrayrulewidth]{1-7}\cmidrule[3\arrayrulewidth]{9-10}
		\end{tabular}
	}
\end{table*}

\begin{table*}[tbh]
	\centering % Comp (dist2), Acc (dist1)
	\caption{\color{blue} Mean of runtime(Second) and memory consumption (GB) during reference on a typical sequence of ScanNet.}
	\label{tab:mem_runtime}
	\resizebox{0.85\textwidth}{!}{
	    \color{blue}
		\begin{tabular}{cccccccC{0.3cm}cc}\cmidrule[3\arrayrulewidth]{1-7}\cmidrule[3\arrayrulewidth]{9-10}
			Method       & MVS Dep. & Feat. Enc.  & Feat. Agg. & 3D SpCNN   & GRU Fusion & Total & &  Kf./Sec.& Memory (GB)\\ \cline{1-7}\cline{9-10}
  	        NeuralRecon \cite{sun2021neuralrecon} & - & 0.037& 0.012 & 0.096 & 0.063 & 0.219& & 41.10 & 0.988 \\
			Ours & 0.375& 0.025& 0.099& 0.060& 0.057& 0.709 & &12.70 & 1.68 \\
			Ours (High Reso) & 0.386& 0.025& 0.573& 0.225& 0.318 & 1.786& &5.04& 9.06 \\
			\cmidrule[3\arrayrulewidth]{1-7}\cmidrule[3\arrayrulewidth]{9-10}
		\end{tabular}
	}
\end{table*}

% 0.384+ 0.025 + 0.181+ 0.573+ 0.225+ 0.315 = 1.703
% 0.377 + 0.025 + 0.061 + 0.099 + 0.060 + 0.057 = 0.679
\begin{table*}[tbh]
	\centering % Comp (dist2), Acc (dist1)
	\caption{Mean of reference runtime (Second) and memory consumption (GB) on a typical sequence of ScanNet.}
	\label{tab:mem_runtime}
	\resizebox{0.85\textwidth}{!}{
		\begin{tabular}{ccccccccC{0.3cm}cc}\cmidrule[3\arrayrulewidth]{1-8}\cmidrule[3\arrayrulewidth]{10-11}
			Method       & MVS Dep. & Feat. Enc. & TSDF-Fusion  & Feat. Agg. & 3D SpCNN   & GRU Fusion & Total & &  Kf./Sec.& Memory (GB)\\ \cline{1-8}\cline{10-11}
  	        NeuralRecon \cite{sun2021neuralrecon} & - & 0.037 & - & 0.012 & 0.096 & 0.063 & 0.219& & 41.10 & 0.988 \\
			Ours & 0.377& 0.025& 0.061& 0.099& 0.060& 0.057& 0.711 & &12.66 & 1.68 \\
			Ours (High Reso) & 0.384& 0.025 & 0.181& 0.573& 0.225& 0.315 & 1.779& &5.06& 9.06 \\
			\cmidrule[3\arrayrulewidth]{1-8}\cmidrule[3\arrayrulewidth]{10-11}
		\end{tabular}
	}
 \vspace{-1em}
\end{table*}
\fi

\begin{table*}[tbh]
	\centering % Comp (dist2), Acc (dist1)
	\caption{Mean of runtime (Second), memory consumption (GB), and number of nonempty voxels in three-level feature volumes, during the reference on a typical sequence of ScanNet.}
	\label{tab:mem_runtime}
	\resizebox{0.95\textwidth}{!}{
		\begin{tabular}{ccccccccC{0.3cm}ccccc}\cmidrule[3\arrayrulewidth]{1-8}\cmidrule[3\arrayrulewidth]{10-14}
			Method       & MVS Dep. & Feat. Enc. & TSDF-Fusion  & Feat. Agg. & 3D SpCNN   & GRU Fusion & Total & &  Kf./Sec.& Voxels L0 & Voxels L1& Voxels L2 & Memory (GB)\\ \cline{1-8}\cline{10-14}
  	        NeuralRecon \cite{sun2021neuralrecon} & - & 0.037 & - & 0.012 & 0.096 & 0.063 & 0.219& & 41.10 & 4307.436 & 11893.692 & 46665.385 & 0.988 \\
			Ours & 0.377& 0.025& 0.061& 0.099& 0.060& 0.057& 0.711 & &12.66 & 1390.744 & 6156.615  & 32336.641 & 1.68 \\
			Ours (High Reso) & 0.384& 0.025 & 0.181& 0.573& 0.225& 0.315 & 1.779& &5.06 & 6962.026 &39470.615 &  230968.897 & 9.06 \\
			\cmidrule[3\arrayrulewidth]{1-8}\cmidrule[3\arrayrulewidth]{10-14}
		\end{tabular}
	}
 \vspace{-1em}
\end{table*}

%\begin{table*}[tbh]
%	\centering % Comp (dist2), Acc (dist1)
%	\caption{Mean of runtime(second) and number of nonempty voxels in feature volumes on Scannet test split.}
%	 Note the memory cosumption here is the allocated memeory. Actually, the reserved memeory are 2.021 (neuralrecon), 3.034 or 3.316 (ours),18.146(ours high)
%	\label{tab:mem_runtime}
%	\resizebox{\textwidth}{!}{
%		\begin{tabular}{cccccccC{0.5cm}ccc}\cmidrule[3\arrayrulewidth]{1-7}\cmidrule[3\arrayrulewidth]{9-11}
%			Method       & MVS Dep. & Feat. Enc.  & Feat. Agg. & 3D SpCNN   & GRU Fusion & Total & & Voxels L0 & Voxels L1& Voxels L2 \\ \cline{1-7}\cline{9-11}
%			NeuralRecon \cite{sun2021neuralrecon} & - & 0.030& 0.028 & 0.035 & 0.023 & 0.299& &7267.57 &15954.09 &58328.85 \\
%						Ours & 0.323& 0.027& 0.035& 0.022& 0.019& 1.253& & 1560.19 & 7669.65& 41094.30 \\
%			Ours & 0.327& 0.027& 0.041& 0.024& 0.020& 1.130 & & 1844.11 &7080.08 & 38330.30 \\
%			Ours (High Reso) & 0.327& 0.027& 0.276& 0.086& 0.128& 3.978& & 10574.00& 58550.53& 334563.45 \\
%			\cmidrule[3\arrayrulewidth]{1-7}\cmidrule[3\arrayrulewidth]{9-11}
%		\end{tabular}
%	}
%\end{table*}


\subsection{Ablation Study}
To examine the effectiveness of our design choices, we conduct ablation studies on the ScanNet dataset at the default resolution. The results are reported in Table~\ref{tab:ablation-3d}. We first examine our method without sparsification. 
%The result is not out of our expectation that disabling the sparsification would taken all the voxels in a dense volume into consideration thus lead to a better reconstruction. However, we can find that ours method with MVS guided sparsified feature volume has very comparable performance to the dense volume method, which demonstrates the applicability of our sparsification choice, which is memory friendly and enables high resolution reconstruction.
%
% In this case, the F-score is a bit higher, while the completeness of the reconstructed mesh is certainly worse. Despite producing a less complete mesh, running our method without the sparsification incurs a higher memory consumption due to more voxels needing to be allocated.
%
In this case, the F-score is a bit higher, while running our method without the sparsification incurs a higher memory consumption due to more voxels needing to be allocated.
%
We further ablate our method by removing the predicted depth uncertainty for feature allocation~-- allocating features within a constant distance of 5 voxels around the surface recovered from the predicted MVS depth. Noticeably, our full method has better performance due to the probabilistic feature allocation accounting for the uncertainty of predicted MVS depth.
%
It is also clear from the table that our choice of feature augmentation using the TSDF values and weights generated from trivial TSDF fusion of MVS depth, as well as our choice of self-attention for feature aggregation, have significant effects on the system performance.
%
The hints from MVS TSDF values and weights can guide the network for better convergence. The attention mechanism for feature aggregation from multiple views enables selectively absorbing informative deep features for 3D structure recovery.
%
For the last ablation study in Table~\ref{tab:ablation-3d}, we investigate whether it is possible to reduce the number of parameters by sharing the feature encoder of the MVS Network with the 2D CNN for feature extraction (see Fig.~\ref{fig:framework}), instead of using separate feature encoders for the two modules in our design choice. Notably, the performance is significantly deteriorated due to the fact that MVS and feature volume fusion \rev{require different features}.

\begin{table}[!t]
	%	\vspace{-1.2cm}
	\centering % Comp (dist2), Acc (dist1)
	\caption{Ablation study: 3D geometry metrics evaluated on ScanNet test split.}
	\label{tab:ablation-3d}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{cccccc}
			\Xhline{3\arrayrulewidth}
			Method       & Comp $\downarrow$ & Acc $\downarrow$   & Recall $\uparrow$ & Prec $\uparrow$   & F-score  $\uparrow$    \\ \hline
			% NeuralRecon \cite{sun2021neuralrecon} & 0.137   & \textbf{0.056}  & 0.470   & \textbf{0.678}  & 0.553  \\
			% Ours (High Reso) & 0.098 & 0.061 &0.552 & 0.666 &0.602 \\
   % Ours (High Reso) & 0.103 & 0.063 & 0.538 & 0.658 & 0.590 \\
   Ours (High Reso) & 0.116 & 0.056 & 0.525 & 0.675 & 0.589 \\
			Ours & 0.110 & 0.058 & 0.505 & 0.665 & 0.572  \\ \hline
			Ours: w/o sparsification & 0.123& 0.047& 0.487&0.713& 0.577 \\
			Ours: w/o depth uncer. &  0.111& 0.061& 0.496& 0.651& 0.561 \\
			Ours: w/o tsdf augment. & 0.120& 0.063& 0.472& 0.637& 0.540 \\
			Ours: w/o attention & 0.119& 0.073& 0.451& 0.592& 0.511\\
			Ours: w/o sep. feat. enc.& 0.121& 0.065& 0.463& 0.625& 0.530 \\
			\Xhline{3\arrayrulewidth}
		\end{tabular}
	}
\vspace{-2em}
\end{table}

\subsection{Limitations and Discussions}
Our proposed method leverages \rev{MVS} depth to guide incremental feature volume-based reconstruction. MVS can provide rough locations of the physical surface and enable sparse allocation, while feature volume-based fusion can further regularize, refine, and denoise the recovered 3D structures from MVS depth. With the MVS guidance, more geometric details can be recovered. However, it pays the cost that local smoothness can be slightly degraded. Since the sparse feature allocation is critical for our proposed method, if the MVS network fails to predict a depth distribution surrounding the true physical surface, the feature volume-based pipeline can not recover appreciable 3D structures from empty voxels.


==> sections_main/05_conclusion.tex <==
%!TEX root = ../main.tex
\section{Conclusion and Future Work}\label{sec:conc}
We presented a real-time incremental 3D dense reconstruction method from monocular videos based on MVS, attention mechanism, sparse 3D CNN, and GRU fusion. Predicted depth maps and uncertainties from MVS neural networks provide an initial guess of the physical surface locations in feature volume. Then feature volume-based pipeline temporally fuses the deep features into the sparsified feature volume to refine 3D geometries and impose local smoothness and 3D priors learned from data. 
The proposed method is demonstrated to perform accurate 3D dense reconstruction on several datasets, and can scale up to high-resolution reconstruction due to its memory-efficient nature in terms of sparse feature allocation. 
%In the future, it is interesting to scale the proposed sparse feature volume-based method to the dense reconstruction of large-scale outdoor scenarios.

\section*{Acknowledgment}
We thank Noah Stier~\cite{stier2021vortx}, Jiaming Sun, and Yiming Xie~\cite{sun2021neuralrecon} for discussions about the evaluations of baselines.
